ALMA Survey of Orion Planck Galactic Cold Clumps (ALMASOP): A Hot Corino Survey toward Protostellar Cores in the Orion Cloud

The presence of complex organic molecules (COMs) in the interstellar medium (ISM) is of great interest since it may link to the origin and prevalence of life in the universe. Aiming to investigate the occurrence of COMs and their possible origins, we conducted a chemical census toward a sample of protostellar cores as part of the ALMA Survey of Orion Planck Galactic Cold Clumps (ALMASOP) project. We report the detection of 11 hot corino sources, which exhibit compact emissions from warm and abundant COMs, among 56 Class 0/I protostellar cores. All the hot corino sources discovered are likely Class 0 and their sizes of the warm region ($>$ 100 K) are comparable to 100 au. The luminosity of the hot corino sources exhibits positive correlations with the total number of methanol and the extent of its emissions. Such correlations are consistent with the thermal desorption picture for the presence of hot corino and suggest that the lower luminosity (Class 0) sources likely have a smaller region with COMs emissions. With the same sample selection method and detection criteria being applied, the detection rates of the warm methanol in the Orion cloud (15/37) and the Perseus cloud (28/50) are statistically similar when the cloud distances and the limited sample size are considered. Observing the same set of COM transitions will bring a more informative comparison between the cloud properties.

==> tab_13C12C.tex <==
\begin{deluxetable}{lccccccccccccccccc}
% \tabletypesize{\large}
\setlength{\tabcolsep}{14pt}
% \renewcommand{\arraystretch}{0.95}
\tablecaption{\label{tab:13C12C} The \CCIso~ratios}
\tablehead{
\tablehead{\colhead{Source} & \colhead{$\frac{[\mathrm{CH_3OH}]}{[\mathrm{^{13}CH_3OH}]}$} & \colhead{$\frac{[\mathrm{OCS}]}{[\mathrm{O^{13}CS}]}$}
}} 
\startdata
G205S1A & 1.6$^{+1.4}_{-0.8}$ & 5.3$^{+3.5}_{-3.6}$ \\
G208N1 & 3.8$^{+0.5}_{-0.5}$ & 4.8$^{+0.7}_{-0.7}$ \\
G211S & 4.5$^{+0.2}_{-0.3}$ & 7.7$^{+1.6}_{-1.7}$ \\
\enddata 
% \tablecomments{
% The sources, where the \CCIso~of OCS and HCCCN are unable to be derived, are not listed.
% Both HCCCN and HC$^{13}$CCN are detected with only one single transition and their \Tex\ is assumed to be 100~K in the XCLASS simulation.
% the \Ntot~may therefore not be properly delivered.
% }
% \tablerefs{
% }
\end{deluxetable}
